Over-the-Air Runtime Wi-Fi MAC Address Re-randomization

Medium Access Control (MAC) address randomization is a key component for privacy protection in Wi-Fi networks. Current proposals periodically change the mobile device MAC addresses when it disconnects from the Access Point (AP). This way frames cannot be linked across changes, but the mobile device presence is exposed as long as it remains connected: all its communication is trivially linkable by observing the randomized yet same MAC address throughout the connection. Our runtime MAC re-randomization scheme addresses this issue, reducing or eliminating Wi-Fi frames linkability without awaiting for or requiring a disconnection. Our MAC re-randomization is practically 'over-the-air': MAC addresses are re-randomized just before transmission, while the protocol stacks (at the mobile and the AP) maintain locally the original connection MAC addresses - making our MAC layer scheme transparent to upper layers. With an implementation and a set of small-scale experiments with off-the-shelf devices, we show the feasibility of our scheme and the potential towards future deployment.

==> section/related.tex <==
\section{Related Works}
\label{sec:related}

Full frame encryption.
